TEngineDB-V: An OLAP-Native Vector Search System for Large-$k$ Workloads at Tencent

Vector search systems are essential infrastructure for modern data-driven applications. Large-$k$ analytical vector search, which retrieves $k=10^3$--$10^5$ results for analytics (e.g., aggregation, filtering, joins), is increasingly important for emerging workloads, including LLM data management and advertising analysis at Tencent. Existing systems remain inadequate: specialized vector databases often cap $k$ (e.g., $k \leq 10^4$) to satisfy tail-latency constraints and offer limited analytical support, while OLAP systems typically embed per-segment vector indexes as black boxes, causing severe read/compute amplification and preventing native query optimization. This paper presents TEngineDB-V, an OLAP-native vector search system for large-$k$ workloads. TEngineDB-V makes vector search a first-class analytical primitive in Tencent's OLAP engine through a global segment-decoupled index materialized as relational tables, eliminating scatter-gather execution, reducing amplification, and enabling native storage optimizations. It decomposes IVFPQ-based search into relational operators, integrates OLAP optimizations, and introduces DPPQ, which combines direction-aware quantization with hierarchical residual refinement to improve recall while preserving relational efficiency. TEngineDB-V further incorporates index-aware query rewriting and a distributed-aware cost model for efficient distributed execution. Experiments show that TEngineDB-V achieves up to a $145\times$ speedup over competitive systems such as StarRocks, and up to a $52\times$ improvement in 10-billion-scale production deployments.

==> Styles/revision.tex <==
\usepackage{tcolorbox}
\tcbuselibrary{breakable}
\usepackage{marginnote}
\usepackage{framed}
\setlength{\FrameSep}{2pt}      % 内容与框线内部的间距（默认6pt）
\setlength{\OuterFrameSep}{-0pt}   % 框线与外部正文的间距（默认

% 定义一个名为 Meta 的盒子环境
\newtcolorbox{MetaBox}{
  breakable,
  colback=green!5,      % 背景色：极浅蓝
  colframe=green!30,    % 边框色：浅蓝
  boxrule=0.5pt,       % 边框宽度
  arc=2pt,             % 圆角
  left=5pt, right=5pt, top=5pt, bottom=5pt, % 内边距
  fontupper=\small % 内部字体：稍小+斜体, \itshape
}

% 定义一个名为 R1 的盒子环境
\newtcolorbox{R1Box}{
  breakable,
  colback=blue!5,      % 背景色：极浅蓝
  colframe=blue!30,    % 边框色：浅蓝
  boxrule=0.5pt,       % 边框宽度
  arc=2pt,             % 圆角
  left=5pt, right=5pt, top=5pt, bottom=5pt, % 内边距
  fontupper=\small % 内部字体：稍小+斜体, \itshape
}

% 定义一个名为 R3 的盒子环境
\newtcolorbox{R3Box}{
  breakable,
  colback=orange!5,      % 背景色：极浅蓝
  colframe=orange!30,    % 边框色：浅蓝
  boxrule=0.5pt,       % 边框宽度
  arc=2pt,             % 圆角
  left=5pt, right=5pt, top=5pt, bottom=5pt, % 内边距
  fontupper=\small % 内部字体：稍小+斜体, \itshape
}

% 定义一个名为 R4 的盒子环境
\newtcolorbox{R4Box}{
  breakable,
  colback=red!5,      % 背景色：极浅蓝
  colframe=red!30,    % 边框色：浅蓝
  boxrule=0.5pt,       % 边框宽度
  arc=2pt,             % 圆角
  left=5pt, right=5pt, top=5pt, bottom=5pt, % 内边距
  fontupper=\small % 内部字体：稍小+斜体, \itshape
}

\definecolor{shadecolor}{rgb}{0.92,0.92,0.92}

\newcommand{\MetaColor}[1]{\textcolor{teal}{#1}}
\newcommand{\RaColor}[1]{\textcolor{blue}{#1}}
\newcommand{\RbColor}[1]{\textcolor{orange!80!black}{#1}}
\newcommand{\RcColor}[1]{\textcolor{red}{#1}}

\colorlet{BLUE}{blue}
\colorlet{ORANGE}{orange!80!black}
\colorlet{RED}{red}
